A Type System for Required/Excluded Elements in CLS

The calculus of looping sequences is a formalism for describing the evolution of biological systems by means of term rewriting rules. We enrich this calculus with a type discipline to guarantee the soundness of reduction rules with respect to some biological properties deriving from the requirement of certain elements, and the repellency of others. As an example, we model a toy system where the repellency of a certain element is captured by our type system and forbids another element to exit a compartment.

==> eptcsdata.tex <==
\providecommand{\event}{S. Barry Cooper \& Vincent Danos (eds.): Fifth Workshop on\\
Developments in Computational Models---Computational Models From Nature}
\providecommand{\volume}{9}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{38}
\providecommand{\eid}{5}

